Unsupervised Discrete Sentence Representation Learning for Interpretable Neural Dialog Generation

The encoder-decoder dialog model is one of the most prominent methods used to build dialog systems in complex domains. Yet it is limited because it cannot output interpretable actions as in traditional systems, which hinders humans from understanding its generation process. We present an unsupervised discrete sentence representation learning method that can integrate with any existing encoder-decoder dialog models for interpretable response generation. Building upon variational autoencoders (VAEs), we present two novel models, DI-VAE and DI-VST that improve VAEs and can discover interpretable semantics via either auto encoding or context predicting. Our methods have been validated on real-world dialog datasets to discover semantic representations and enhance encoder-decoder models with interpretable generation.

==> backup.tex <==
Converse like human is very challenge because it involves in complex decision-making process and involve in knowledge from both the discourse history, but also many other factors, such as speaker personal characteristics, conversation environment and etc. Therefore, only having the discourse history (sometimes even a clipped one) will results into a one-to-many problem. Or more specfically, $P(X|C)$ can be highly complex multi-modal distribtion. In the last few years, researchers have discovered that properly modeling the distribution of latent variable of a conversation is the principle method to capture the distribution of valid responses given a windowed discourse history. Building upon the past discovery, this study first time categorize the latent variables into several groups, and then propose a general framework for learning differnet types of latent variables. Then we also presented two new datasets that are designed to benchmark the performance of neural conversation models in terms of: 1. the ability of learning accurate aggreagted posterior distribution 2. the ability of recovering latent variables into dense embedding space with meanifuling grouping. We show that our proposed model achieves the state-of-the-art performance on the proposed benchmark. Moreover, a extra benefit of the proposed model is that it can be also used to measure the degree of diversity in a new conversation corpus, after proven its' ability of learning the diversity in our benchmark dataset. 

Modeling dialog can be formalized as the desnsity estimation of $P(X|C)$ where X is a sequence of word tokens. The state-of-the-art results have been achieved via using auto regressive models, e.g. RNN to model the conditional distribution of $P(w_{t+1}|w_{<t+1}, c)$. Recent work of Mixture of Softmax fix the low-rank issue of standard softmax and push the expressiveness even further. Therefore, if one only wants to estimate the conditional distribution of resposnes given context, auto regressive models in theory is sufficient to achieve the task. On the other hand, one property of auto regressive model, e.g. seq2seq is that is maintain a dense representation inside and only outputs the final probability distribution in the end via softmax or mixture of softmax. As a results, all of the factors accounted for variability of the next word is mixed together in the final outputs. This property however is not deseriable in developing conversatioal agents, where naturally we wish to learn hierarhical process so that the variabituy of the next action/topic is sperated from the lexical choice variabitlty given that other high-level factors are already chosen. Another motivation of learning hierarthiacal process is that it opens the chance for optimizing systems' discourse-level decision making via reinforcement learning or enable policy adaption to new domains while the low level process (i.e. referred as the NLG component in the dialog community) remains the same. Therefore, this study strives to unsupervisedly recover such hierarchical process of dialog data, which results into better system perforamnce and interpretabiltiy. 



\section{Proposed Methods}
The basic idea of LAM is to optimize the following objective 
\begin{equation}
    \mathcal{L}=logP_{z\sim q(z|x)}(x|z) + D(q(z),p(z|c))
\end{equation}
The key design choice is here the type of recognition network $q(z|x)$ and the type of distance function we choose $D(q, p)$. Many options are avaliable. For the recognition network, the options explored here are:
\begin{enumerate}
    \item Deterministic Continuous Mapping: Autoencoder
    \item Deterministic Discrete Variable: VQ-VAE
    \item Stochastic Continuous Mapping: VAE single Gaussian
    \item Stochastic Discrete Mapping: Gumbel-VAE
\end{enumerate}

On the other hand, we deploy two strategies for modeling the prior network, which should be expressive enough to approxmiate complex multi-modal distribution.
\begin{enumerate}
    \item Softmax output for discrete codes. With LSTM to take into latent account??
    \item GAN for continuous codes.
\end{enumerate}
Now we need to think of the pros and cons of each type of encoding.

\subsection{Fine Tunning Decoder}
Since the decoder is trained to read in the latent sample from the recognition network, but in testing it uses the sample from the prior network. This discremency may lead to undesired bevhaior. Therefore, we siwtch the sample from recogntion network to prior network with probabiltiy controlled by x, which is similar to the scheduling smapling algorihtm proposed in[]. However we do this at sequence level instead of word level.

\section{Discussions}
We can express the conditional probability as follows:
\begin{align}
    P(x|c) & = E_{z\sim Q(z)}log(P(x|z)\\
    & + D_{KL}(Q(z), P(z|c)) \\
    & + D_{KL} (Q(z), P(z|c,x))
\end{align}
In the standard encoder decoder training, $Q(Z)=Q(Z|C)$, where $Q(Z|C)$ is the encoder. Then the conditional likelihood becomes:
\begin{align}
    P(x|c) & = E_{z\sim Q(z)}log(P(x|z)\\
    & + D_{KL} (Q(z|c), P(z|c,x))
\end{align}
The corresponding variational lower bound is tight if $D_{KL} (Q(z|c), P(z|c,x))=0$, so that we can assume $P(z|c)=P(z|c,x)$. If we assume a joint probability to be: $P(x, y, z) = P(x|z)P(z|c)P(c)$, then we can have:
\begin{align}
    P(z|x,c) &= \frac{P(z|c)P(x|z)}{P(x|c)} = P(z|c)\\
    P(x|c)  & = P(x|z)\\
    P(z|c)P(x|z) &= P(z|c)P(x|c)\\
    P(x,z|c) &= P(x|c)P(z|c)
\end{align}
Therefore, the lower bound is only tight if $Z$ and $X$ are conditional independent with each other given a context $c$.


Regularization


sys-greeting       & Hello, welcome to the Cambridge ...      \\
sys-thanks         & You are welcome      \\
sys-request        & What kind of food do you like?      \\
sys-confirm        & can you please repeat that?      \\
usr-inform         & Chinese food in the west part of town     \\
usr-request-detail & Can I get the phone number?     \\ 
usr-yn-answer      & it doesn't matter               \\ 
usr-request        & I want a Turkish restaurant      \\ \hline
\multicolumn{4}{c}{DSTC} \\\hline
sys-greeting       & Hello, welcome to the Cambridge ...      \\
sys-thanks         & You are welcome      \\
sys-request        & What kind of food do you like?      \\
sys-confirm        & can you please repeat that?      \\
usr-inform         & Chinese food in the west part of town     \\
usr-ask-detail     & Can I get the phone number?     \\ 
usr-yn-answer      & It doesn't matter               \\ 
usr-request        & I want a Turkish restaurant      \\ \hline



\begin{table}[ht]
\centering
\begin{tabular}{l|l|lll}\hline
Domain & Model        & PPL       & $\text{KL}(q\|p)$ & $I(x,z)$   \\ \hline
PTB    & RNNLM        & 45.51     & -                 & -          \\
       &              & 116.22    & -                 & -          \\ \hline
       &  AE          & 20.70     & 0.308             & 1.45       \\
       &              & 66.49     & 2.20              & 0.349      \\ \hline
       & DVAE*        & 37.20     & 0.036             & 0.534      \\ 
       &              & 70.84     & 0.315             & 0.286      \\ \hline      
       & DI-VAE       & 21.84     & 0.068             & 1.16       \\ 
       &              & 52.53     & 0.133             & 1.18         \\ \hline
\end{tabular}
\label{tbl:vae-main}
\caption{Comparison of various discrete sentence representations. VAE* refers to training Discrete VAE with special tricks described in Section~\ref{sec:exp_setup}.}
\end{table}


\begin{table}[ht]
\centering
\begin{tabular}{llllll}\hline
K-M     & $K^M$       & PPL       & $\text{KL}(q\|p)$ & $I(x,z)$ \\ \hline
1000-1  & 1000        & 47.92     & 0.074             & 0.957     \\
10-3    & 1000        & 40.01     & 0.069             & 1.105     \\
4-5     & 1024        & 35.75     & 0.070             & 1.075     \\ 
2-10    & 1024        & 34.60     & 0.020             & 0.637     \\ \hline
\end{tabular}
\label{tbl:vae-size}
\caption{DI-VAE on PTB with different dimension shape under the same budget.}
\end{table}


\begin{table}[ht]
\centering
\small
\begin{tabular}{p{0.07\textwidth}|p{0.1\textwidth}|p{0.23\textwidth}}\hline
\textbf{Model-Domain}    & \textbf{Action Name}        & \textbf{Sample utterance}   \\ \hline
DI-VAE sw   & opinion            & - I don't think there is a solution. \\ 
             &                    & - I'd like to stay home for a while but \\\cline{2-3}
             & affirm             & - oh yeah                \\
             &                    & - oh I see                 \\ \hline
DI-VST sw   & topic opener       & - well how long have you been here   \\
             &                    & - I have a sister in New Mexico \\ \cline{2-3}
             & back-channel       & - Oh yeah                   \\ 
             &                    & - um-hum                  \\\hline
DI-VAE smd & confirm info       & - you are looking for a British restaurant, right?                \\
             &                    & - you are looking for a Italian restaurant, right? \\ \cline{2-3}
             & ask detail         & - can I have the price range? \\ 
             &                    & - can I have the phone number? \\ \hline  
DI-VST smd & open request       & - hi I am looking for a restaurant.                \\
             &                    & - can I get a restaurant in the center of town?\\ \cline{2-3}
             & give info          & - Chinese food. \\ 
             &                    & - I need Jamaican food. \\ \hline           
\end{tabular}
\label{tbl:code-meaning}
\caption{Example latent actions discovered in SW and DSTC using our methods.}
\end{table}

\subsection{Conditional or Marginal Mutual Information?}
A natural alternative is to maxmize $I(Z,X|C)$ instead of $I(Z, X)$. A similar derivation will show that the regurlzation term $\text{KL}(q(z_{c}|x)|p(z_{c}|c))$ can also be broken down into $I(Z,X|C)+\text{KL}(q(z|c)|p(z|c))$. Therefore, the proposed loss funciton is in fact trying to reduce the conditional mutual information. At first glance, this might be harmful for learning latent $z$. We here argue that it is correct to maxmize $I(X, Z)$ instead of $I(X,Z|C)$. The reason can be seen by rewrite the conditional mutual information as $I(Z,X|C)=-H(Z|X,C)+H(Z|C)$. This means that maximum $I(X,Z|C)$ leads to a uniform conditional distribution $P(Z|C)$ and very peaky posterior $P(Z|X,C)$. The problem lies in maxmizing $H(Z|C)$, because that means $P(Z|C)$ will be uniform for any dialog context. THis effectively makes model to bestow a different meaning for $z$ depends on the context. On the other hand, we wish to learn a latent representation $z$ that has consistent semantics for all context. On the other hand, maximizing $I(X,Z)$ only results into uniform $P(Z)$ and freely allows $P(Z|C)$ to have low entropy.



==> intro-back.tex <==
The generative neural dialog model is one of the most prominent frameworks for developing conversational agents in complex domains. The base model is the neural encoder decoder models~\cite{vinyals2015neural} widely used for various types of conditional text generation, e.g. machine translation~\cite{cho2014learning}. The basic idea is to use a encoder network transform the dialog context $c$ into distributed vectors and then a decoder network is used to generate the system's next response $x$. The encoder and decoders can then be trained jointly by maximizing the conditional probability $p(x|c)$. Past research has shown that Recurrent Neural Network (RNN) decoders can achieve strong performance in modeling complex distribution over text~\cite{oord2016pixel,lu2016knowing} and substantial effort has been invested to improve the expressiveness of RNNs~\cite{bahdanau2014neural,zhang2016highway,yang2017breaking}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.43\textwidth]{figures/goal.png}
    \caption{Our proposed models learn sentence-level discrete latent actions for interpretable conditional text generation.}
    \label{fig:goal}
\end{figure}
This paper begins with a different question: \textit{``Is a perfect model for $p(x|c)$ all we need for future dialog agents?''} Prior research in dialog systems have stressed the importance of learning a hierarchical decision-making process where a dialog manager first decides high-level actions and then a natural language generator produces the response~\cite{litman1987plan,raux2005let}. This hierarchical generation process is attractive because it provides interpretable representations about a system's intentions. Unfortunately, for generative neural dialog models, such information is hidden inside the distributed representation and the decoders only output meaningful symbols at the word-level. Thus it has been challenging to understand the behavior of a neural dialog model.

This paper strives to improve neural dialog systems by introducing high-level actions into encoder-decoder models in an unsupervised fashion. The basic idea (Figure~\ref{fig:goal}) is to learn a set of latent variables $z$ (referred as \textit{latent actions}) that capture sentence-level features of the response $x$. For given a context $c$, the model will first predicts the latent actions and then generates $x$ using information from both $z$ and $c$. Moreover, our proposed methods are unsupervised so that it can easily scale up to large datasets in new domains to discover features about $x$ that are not feasible before. Whereas the prior work in augmenting neural dialog models with extra features have used hand-crafted actions, e.g. dialog acts or topics~\cite{xing2016topic}, which are domain dependent and are often difficult to transfer to new situations~\cite{margolis2010domain}. 

Specifically, we focus on developing discrete sentence representation using rich learning signals, including auto-encoding and context predicting. We found a simple combination of sentence variational autoencoders (VAEs)~\cite{bowman2015generating} and Gumbel-Softmax Trick~\cite{jang2016categorical,maddison2016concrete} fails to learn meaningful discrete representations. We then highlight the anti-information limitation of evidence lowerbound objective (ELBO) in VAE and improve it by proposing Discrete information VAE (infoVAE) that maximize the mutual information between data and latent actions. The proposed objective is then used to extend Skip Though~\cite{kiros2015skip} to Discrete information Variational Skip Thought (infoVST). Both models significantly outperform the standard VAEs in terms of representation learning and text generation. We finally present how the learned latent actions can be integrated with any encoder decoder models. The proposed systems are tested on both task and chat-oriented real-world dialog datasets. Experiments showed that the two proposed methods can discover meaningful yet different latent actions from unlabelled data. 

In the rest of paper, we begin with an review about the related work, noting their need for supervised labels to achieve interpretable dialog generation. Then we describe the proposed architecture and methods. Finally, our methods were tested on several real-world conversational datasets using both automatic and human evaluations.
